Morph: Flexible Acceleration for 3D CNN-based Video Understanding

The past several years have seen both an explosion in the use of Convolutional Neural Networks (CNNs) and the design of accelerators to make CNN inference practical. In the architecture community, the lion share of effort has targeted CNN inference for image recognition. The closely related problem of video recognition has received far less attention as an accelerator target. This is surprising, as video recognition is more computationally intensive than image recognition, and video traffic is predicted to be the majority of internet traffic in the coming years. This paper fills the gap between algorithmic and hardware advances for video recognition by providing a design space exploration and flexible architecture for accelerating 3D Convolutional Neural Networks (3D CNNs) - the core kernel in modern video understanding. When compared to (2D) CNNs used for image recognition, efficiently accelerating 3D CNNs poses a significant engineering challenge due to their large (and variable over time) memory footprint and higher dimensionality. To address these challenges, we design a novel accelerator, called Morph, that can adaptively support different spatial and temporal tiling strategies depending on the needs of each layer of each target 3D CNN. We codesign a software infrastructure alongside the Morph hardware to find good-fit parameters to control the hardware. Evaluated on state-of-the-art 3D CNNs, Morph achieves up to 3.4x (2.5x average) reduction in energy consumption and improves performance/watt by up to 5.1x (4x average) compared to a baseline 3D CNN accelerator, with an area overhead of 5%. Morph further achieves a 15.9x average energy reduction on 3D CNNs when compared to Eyeriss.

==> outline.tex <==
Paragraph 1:
- 2D CNNs have been very successful, which has spurred many designs and use cases 
- People are building HW accelerators for 2D

Paragraph 2:
- Similar trend now happening for video
- we make an observation that: best algorithm is 3D CNN
- Brief description of 3D CNN
- 3D CNN extremely compute intensive --> need HW acceleration to be practical for real time.

--- Challenge ---
Paragraph 3:
- Important to ask: can 3D be trivially implemented with 2D accelerators? 
- No.  Their control logic is not aware of temporal reuse, and thus tiling techniques do not take advantage of the time dimension.  Effectively, running a 3D CNN on a stock 2D accelerator would entail treating the 3D convolution as multiple 2D convolutions, which requires a large number of unnecessary reads from DRAM.
- We make a key observation that several
aspects of 2D CNN design are amplified in 3D CNN

1.) Naive vs. intelligent reuse (???)
2.) Network activations/filter sizes (same as current Fig 1a but with SoA networks --- need to discuss which to show)
3.) Halo \% vs. tile size (y axis: \% redundant reads; x axis tile size; different lines: 2D and 3D)
4.) Compute-boundness (y axis: # MACCs vs. bytes in DNN; x axis: different layers; different lines: different DNNs)

* Network shape changes more dramatically from layer to layer in 3D CNN than in 2D CNN
* Effect of halos is exacerbated in 3D CNN.
-> need bigger tile size to offset halo cost
-> more energy in the common case
-> more levels of hierarchy
* 3D CNN is more on-chip energy bound than 2D CNN. --> managing buffers efficiently more important.
* 

--- This paper ---

Contributions:
* Design the first HW accelerator for 3D CNN called Morph.  Based on the above analysis, our focus 


* Provide thorough comparison between 2D and 3D CNNs in terms of their compute and storage characteristics, as well as a study showing 3D CNN's sensitivity to loop order, tile size, ...
* Evaluation: compare to Eyeriss, etc., MORPH-base.


==> scratch.tex <==

\section{Introduction}
\label{sec:intro}

%% Paragraph 1: Cloud computing promise -- boilerplate.
Cloud computing is a paradigm, ever growing in popularity, that offers on-demand compute and storage resources for users. 
Applications such as machine learning, AI, analytics, web, and mobile services are now frequently hosted in public clouds. 
Protecting users' data in these environments is challenging due to their underlying complexity and shared infrastructure model. 
As a result, multiple attack vectors from infrastructure and service providers, other users, and targeted adversaries remain open. 

%% Paragraph 2: Cloud computing in the past
%%
%\cnote{TXT intro less important now that we de-emph obliviousness}
Up until recently, secure cloud computing could only be achieved through cryptography (e.g., fully homomorphic encryption -- FHE~\cite{Gentry2009}), or through course-grained hardware isolation techniques (e.g., Intel TPM+TXT~\cite{IntelTXT,McCune2008,TPMspec1}).
Both of the above have severe performance and usability limitations. 
FHE, for example, introduces many orders of magnitude overheads.
On the other hand, these techniques provide very strong security guarantees (stronger than TPM+TXT) needed for applications
that operate over highly sensitive data (e.g., federal, military, government data, etc.). They can be used to protect even against 
malicious operating systems snooping on the data access-pattern. 
%TPM+TXT runs code on bare hardware, yet incurs very high switching cost in/out of TXT and low hardware utilization since the secure application owns the entire machine. 
%% Paragraph 3: SGX, cloud computing today
%%

Recently, Intel released an instruction set extension called \emph{Software Guard Extensions} (SGX) which addresses the above performance challenges~\cite{sgxexplained,SGX2,SGX1}.
In SGX, user-level sensitive portions of ring-3 applications can be run in one or more application containers called enclaves.
While running, SGX uses a set of hardware mechanisms to preserve the privacy and integrity of enclave memory.
However, using SGX to achieve whole-program privacy against software adversaries still faces multiple challenges.
First, the user must map its application to enclave(s) in a way that gives the best trade-off in trusted computing base (TCB) size, performance and code isolation.
The default approach, natively supported by Intel SGX, is to manually partition the application into trusted and untrusted code~\cite{panoply,opaque}. 
This is non-trivial: code within enclaves is trusted and enclaves have limited functionality (e.g., no support for IO/syscalls and a bounded memory size).
Alternatively, a number of works study how to load unmodified applications into enclaves~\cite{scone,baumann2015shielding,ryoan,graphene}.
While more automated, these approaches require a larger TCB.
Second, the user must carefully write enclave code to avoid numerous software side-channels~\cite{Brasser,lee2016inferring,SchwarzWGMM17,wang2017leaky,xu2015}.
%Due to the architectural limitations and security weaknesses (such as lack of access-pattern protections),  how to build applications 
%
%Further, a change to any part of the application requires the vendor to re-compile and re-certify the application.
Taken together, leveraging SGX to achieve small TCB, side channel-free trusted execution environments remains an open problem.

%% Part 2:
%Second, as it time-shares the CPU with other applications and privelaged code, SGX can leak sensitive data over covert channels (e.g., cache/branch predictor sharing, page fault pattern).
%Researchers have shown how these indirect leakages can be devastating -- from leaking key material~\cite{} to the outlines of sensitive images~\cite{}.
%Prior work propose to transform the whole program to an \emph{oblivious form}~\cite{Raccoon,ConstantTimePrograms,CiteTheoryOnObliviousness}.
%The downside to obliviousness is performance overhead: conceptually, the program is converted to straight-line code.
%To exacerbate the overhead, prior work has only studied obliviousness as applied to the whole program -- analogous to porting the entire application to a single enclave as described above.

\subsection{This Work}

%% Paragraph 6: Our approach
%%
We address this challenge by designing and implementing $\OSN$ -- an oblivious library enabling applications to be built out of fine-grained building-blocks at the application's data-structure interface boundary. 
Any operation on the data stored by the library is protected using SGX enclaves and remains secure against all software attacks, including all known side-channels. 

Partitioning applications at the oblivious data-structure boundary hits a sweet spot for several reasons.
First, the data-structure interface is narrow, which makes it easier to sanitize application to data-structure requests---improving intra-application security.
Second, the data-structure interface is re-usable across many applications.
A service provider can pre-package data-structure backends as pre-certified blocks with a common interface, enabling application developers to build complex applications from known-good pieces. 
Lastly, each data-structure can seamlessly support multiple clients and can be oblivious to where each client is physically running. 
For the latter point, clients can attach to data-structure enclaves remotely, providing performance improvements to related systems (e.g., oblivious file servers; c.f. Section~\ref{sec:remote_block_store}).

%Further, there is a rich literature in the security community on how to efficiently achieve various security properties when working with various data-structures~\cite{PoR,ORAM,obliDataStruct,Zahur2013}.
%These works can be dropped into our system as different backend implementations, which gives clients the ability to hot-swap between implementations, depending on the application's security requirements.

As part of this research, \emph{we implement and evaluate the first oblivious memory controller running on a real secure hardware platform.}
Our memory controller, which implements an Oblivious RAM (ORAM) protocol~\cite{ORAM}, can be called as a subroutine in a larger application and defends against any active software adversary.
A key insight that drives our design is that with SGX, ORAM state \emph{can safely live anywhere in the system} (e.g., cache, DRAM, disk, etc), even outside the SGX enclave, despite the adversary running concurrent to the victim and controlling the software stack.
For data inside enclaves, the SGX mechanism prevents direct inspection of data.
Thus security against software attacks reduces to accessing in-enclave data in a data oblivious fashion~\cite{ORAM,molnar2005,oml,Raccoon}.
For data living outside enclaves, enclave code can add a second layer of protection (via encryption, integrity checks, etc) to extend the trust boundary.

%Our system's core component is a fully-implemented SGX-based secure memory controller that exposes a block $\mathsf{read}(\mathsf{addr})$ and $\mathsf{write}(\mathsf{addr}, \mathsf{data})$ interface to applications.
%This memory controller runs in software, partly in an SGX enclave and partly in outside ring-3 support logic.
%The controller's primary design consideration is \emph{flexibility}: we wish for the core controller to be usable across a variety of threat and usage models.
%At the highest level of security, the controller hides which operations it is issued by the user and the arguments issued to those commands. 
%That is, it runs \emph{obliviously}~\cite{ORAM,molnar2005,oml,Raccoon}.
%The module can be parameterized to defend against several types of adversaries, where the highest level of security provides obliviousness (privacy) and integrity (authenticity and freshness) guarantees against \emph{arbitrary software-based} adversaries. 
%The core can be parameterized to defend against a subset of these threats, depending on the context.
%To maximize usability, our controller exposes a low-level and generic `frontend' secure channel-like interface to applications.
%The controller's backend interacts directly with untrusted, available DRAM and/or HDD/SSD storage, in a fashion transparent to the application.
%%Depending on the security level and memory capacity requested requested, the controller runs an Oblivious RAM (ORAM) protocol over untrusted memory for performance~\cite{}.
%
%Building an efficient memory controller in SGX is non-trivial, presenting security and performance challenges, due to the nature of SGX.
%First, despite isolating enclave virtual memory from direct inspection, SGX can leak sensitive data over covert channels (e.g., cache/branch predictor sharing, page fault pattern).
%We employ additional mechanisms (e.g., \cite{molnar2005,oml,Raccoon}) to prevent these leakages.
%Second, SGX enclaves do not support direct IO to disk.
%To support disk backend storage, we partition the controller between trusted and un-trusted zones in a secure fashion.
%Third, SGX does not support persistent integrity across boots, and risks memory controller data corruption on sudden/un-expected shutdowns.
%We develop a novel protocol to make the core memory controller fault tolerant: allowing the controller to quickly and securely recover from such a shutdown or failure (even in the event of partial data loss).
%On the performance front, the whole system design requires a careful balance of resources between enclave memory, untrusted DRAM and untrusted disk(s).
%We propose optimizations to efficiently make use of these different resources in a way that preserves the module's security guarantee.
 
%Using our core memory controller as a building-block, we implement a library of data-structures that can interface directly with applications.
%We evaluate several common data-structures including arrays, sets, dictionaries and lists.
%We further optimize these data-structures to be asymptotically efficient, using techniques from~\cite{ODS}.\cnote{do we have any techniques they don't use}


%Based on our results, we establish a few possible instantiations of our controller
%that may be adjusted depending on the workload to optimize performance. We observe in our evaluation that the performances of these oblivious schemes differ from what may be expected when instantiated within SGX due to limitations of the SGX architecture. Below, we summarize some design choices and challenges 
%that were taken into consideration while building $\OSN$. 
%

\subsection{Contributions}
\noindent This paper makes the following contributions.
\begin{enumerate}
    \item   We design and build an oblivious memory controller from Intel SGX.  
            To the best of our knowledge, the core memory controller (the bulk of our system) is the first oblivious memory controller implemented on a real secure hardware platform.
            We provide two implementations, one using Path ORAM~\cite{pathoram} and one using Circuit ORAM~\cite{Wang2015} and compare both across multiple backend memory organizations (DRAM, SSD and HDD).
            All designs protect against an active software adversary and provide secure fault-tolerance across asynchronous SGX enclave terminations (a common challenge for SGX applications).  
            These extensions may be of independent interest.
    \item   We design and implement $\OSN$, an application library for serving data-structures obliviously in an SGX environment that runs on top of our memory controller.
    \item   We evaluate system performance for $\OSN$ as a stand alone oblivious memory controller and for plug-and-play data structures on an SGX-enabled Dell Optiflex 7040.
            Our system can make oblivious read and write calls to 1~KB memory locations on a 10~GB dataset in 3.4~ms. 
            In the plug-and-play setting, $\OSN$ can make oblivious read and write calls at 8~B granularity on an $80$ MB array in $~1.2$ ms.
            \chris{open source}
        % We additionally provide micro benchmarks of various components, as well as end-to-end performance of the entire system running in the strongest security level (oblivious against and active adversary). 
\end{enumerate}

\subsection{Paper Organization} 
In Section~\ref{sec:model}, we describe our usage and security models.
Section~\ref{sec:prelims} gives a required background on Intel SGX and ORAM. 
Section~\ref{sec:architecture} we give details on our architecture; including the instantiation process, client and server components, optimizations and security analysis.
Section~\ref{sec:integrity} gives a scheme to achieve persistent integrity and fault tolerance.
Section~\ref{sec:impl} describes our prototype implementation and evaluation. 
Section~\ref{sec:related} gives related work, and finally Section~\ref{sec:conclusion} concludes. 







